Towards Refinable Choreographies

We investigate refinement in the context of choreographies. We introduce refinable global choreographies allowing for the underspecification of protocols, whose interactions can be refined into actual protocols. Arbitrary refinements may spoil well-formedness, that is the sufficient conditions that guarantee a protocol to be implementable. We introduce a typing discipline that enforces well-formedness of typed choreographies. Then we unveil the relation among refinable choregraphies and their admissible refinements in terms of an axiom scheme.

==> eptcsdata.tex <==
\providecommand{\firstpage}{61}
\providecommand{\publicationstatus}{J. Lange, A. Mavridou, L. Safina, A. Scalas (Eds.):\\
13th Interaction and Concurrency Experience (ICE 2020).\\
EPTCS 324, 2020, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.324.6}{10.4204/EPTCS.324.6}}


==> ggmacros.tex <==
\usepackage{listings}
\usepackage{mfirstuc}
\usepackage{xstring}
\newif\ifcp
\cpfalse


%%%%%
%% Extensible dashed arrow
%%%%%
\makeatletter
\newcommand*{\da@rightarrow}{\mathchar"0\hexnumber@\symAMSa 4B }
\newcommand*{\da@leftarrow}{\mathchar"0\hexnumber@\symAMSa 4C }
\newcommand*{\xdashrightarrow}[2][]{%
  \mathrel{%
    \mathpalette{\da@xarrow{#1}{#2}{}\da@rightarrow{\,}{}}{}%
  }%
}
\newcommand{\xdashleftarrow}[2][]{%
  \mathrel{%
    \mathpalette{\da@xarrow{#1}{#2}\da@leftarrow{}{}{\,}}{}%
  }%
}
\newcommand*{\da@xarrow}[7]{%
  % #1: below
  % #2: above
  % #3: arrow left
  % #4: arrow right
  % #5: space left 
  % #6: space right
  % #7: math style 
  \sbox0{$\ifx#7\scriptstyle\scriptscriptstyle\else\scriptstyle\fi#5#1#6\m@th$}%
  \sbox2{$\ifx#7\scriptstyle\scriptscriptstyle\else\scriptstyle\fi#5#2#6\m@th$}%
  \sbox4{$#7\dabar@\m@th$}%
  \dimen@=\wd0 %
  \ifdim\wd2 >\dimen@
    \dimen@=\wd2 %   
  \fi
  \count@=2 %
  \def\da@bars{\dabar@\dabar@}%
  \@whiledim\count@\wd4<\dimen@\do{%
    \advance\count@\@ne
    \expandafter\def\expandafter\da@bars\expandafter{%
      \da@bars
      \dabar@ 
    }%
  }%  
  \mathrel{#3}%
  \mathrel{%   
    \mathop{\da@bars}\limits
    \ifx\\#1\\%
    \else
      _{\copy0}%
    \fi
    \ifx\\#2\\%
    \else
      ^{\copy2}%
    \fi
  }%   
  \mathrel{#4}%
}
\makeatother

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%                            ChorGrapm macros                           %%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \def\colorPtp{\color{ForestGreen}}
% \def\colorSbj{\color{ForestGreen}}
% \def\colorAct{\color{ForestGreen}}
% \definecolor{light-gray}{gray}{0.5}
% \def\colorNode{\color{light-gray}}
% \def\colorFun{\color{ForestGreen}}
% \def\colorR{\color{Dandelion}}
% \def\colorE{\color{Dandelion}}
%\definecolor{BrickRed}{rgb}{.8,.25,.33}
%\definecolor{ForestGreen}{rgb}{.0,.27,.13}

\newcommand{\fillcolor}{orange!5}
\def\colorPtp{\color{blue}}
%\def\colorSbj{\color{NavyBlue}}
\def\colorFun{\color{NavyBlue}}
\def\colorAct{\colorFun}
\def\colorOp{\color{OliveGreen}}
\def\colorNode{\color{cyan}}
\def\colorR{\color{OliveGreen}}
\def\colorE{\color{orange}}
\def\sysColor{\color{MidnightBlue}}
\def\ptypeColor{\color{Green}}
\def\ctypeColor{\color{Cyan}}
\def\procColor{\color{MidnightBlue}}
\def\colorMsg{\color{BrickRed}}
\def\contrColor{\color{Plum}}
\newcommand{\cmdcol}{black!30!red!80}
\newcommand{\filecol}{blue}
\newcommand{\nontermcol}{black}
\newcommand{\grsymcol}{ForestGreen}
\newcommand{\keywordcol}{ForestGreen!100!blue!80}

\newcommand{\id}[1][id]{\ensuremath{\mathsf{#1}}}
\newcommand{\keyword}[1]{\textcolor{\keywordcol}{\textsf{#1}}}
\newcommand{\grsym}[1]{\textcolor{\grsymcol}{{#1}}}
\newcommand{\nonterm}[1]{\textcolor{\nontermcol}{\textsl{#1}}}

\newcommand{\toolidcol}{red!10!blue!90}
\newcommand{\toolid}[1]{\textcolor{\toolidcol}{\textbf{\textsf{#1}}}}
\newcommand{\gmc}{\toolid{gmc}}
\newcommand{\sysparser}{\toolid{SystemParser}}
\newcommand{\TS}{\toolid{TS}}
\newcommand{\rep}{\toolid{Representability}}
\newcommand{\bp}{\toolid{BranchingProperty}}
\newcommand{\hkc}{\toolid{hkc}}
\newcommand{\petrify}{\toolid{petrify}}
\newcommand{\bg}{\toolid{BuildGlobal}}

\newcommand{\flag}[1]{\texttt{-{#1}}}
\newcommand{\chosyncmd}[1]{\textcolor{\cmdcol}{\textsf{#1}}}
\newcommand{\chosynfmt}[1]{\textcolor{\cmdcol}{\textsl{#1}}}
\newcommand{\chosynfile}[1]{\textcolor{\filecol}{\textsf{#1}}}

\newcommand{\chorgramsite}{\url{https://bitbucket.org/emlio_tuosto/chorgram/wiki/Home}}
\newcommand{\chorgram}{\toolid{ChorGram}}

\newcommand{\gghide}[2]{{#1} \setminus {#2}}

\newcommand{\msg}[1][m]{\mathsf{\colorMsg{#1}}}
\newcommand{\msgset}{\mathcal{M}}
\newcommand{\chset}{\mathcal{C}}
\newcommand{\events}{\mathcal{E}}
\newcommand{\cfsmevents}{\mathcal{L}}
\newcommand{\lset}{\mathcal{L}}
\newcommand{\gset}{\mathcal{G}}
\newcommand{\inevents}{\events^{\iact}}
\newcommand{\outevents}{\events^{\oact}}

\newcommand{\ptp}[1][A]{\ensuremath{\mathsf{\colorPtp{\capitalisewords{#1}}}}}
\newcommand{\aptp}[1]{\ptp[#1]}
\newcommand{\p}{\ptp}
\newcommand{\q}{{\ptp[B]}}
\newcommand{\s}{{\ptp[S]}}
\newcommand{\rr}{{\ptp[R]}}

\newcommand{\sender}[1][\ae]{\mathsf{\colorPtp{sndr(#1)}}}
\newcommand{\receiver}[1][\ae]{\mathsf{\colorPtp{recv(#1)}}}
\newcommandx{\ggcommon}[3][1=\ptp,2={\aH},3={\aH'},usedefault=@]{f_{#1}}
\newcommandx{\opair}[2][1={\ae},2={\ae'},usedefault=@]{\conf{{#1},{#2}}}
\newcommandx{\hopair}[2][1={\aE},2={\aE'},usedefault=@]{\llparenthesis\, {#1},{#2}\, \rrparenthesis}
\newcommandx{\wf}[2][1={\aG},2={\aG'},usedefault=@]{wf({#1}, {#2})}
\newcommandx{\wb}[2][1={\aG},2={\aG'},usedefault=@]{wb({#1}, {#2})}
\newcommandx{\ws}[2][1={\aG},2={\aG'},usedefault=@]{ws({#1}, {#2})}
\newcommandx{\widx}[2][1={\aW},2={i},usedefault=@]{{#1}[{#2}]}
\newcommandx{\outop}[2][1=\gname,2={}]{{\colorOp{!}}^{{#1}{#2}}}
\newcommandx{\inop}[2][1=\gname,2={}]{{\colorOp{?}}^{{#1}{#2}}}
\newcommandx{\aout}[5][1={\p},2={\q},3=\gname,4=m,5={},usedefault=@]{
  \achan[#1][#2] \outop[{#3}] {\msg[{#4}]}{#5}
}
\newcommandx{\ain}[5][1={\p},2={\q},3=\gname,4=m,5={},usedefault=@]{
  \achan[#1][#2] \inop[{#3}] {\msg[{#4}]}{#5}
}
% \newcommandx{\ain}[5][1={\p},2={\q},3=\msg,4={},5=\gname,usedefault=@]{
%   {#1}{#4} {#2}{#4} \inop[{#5}] {#3}{#4}
% }
\newcommandx{\adep}[1][1={}]{
  \conf{ \aout[@][@][@][@][{#1}], \ain[@][@][@][@][{#1}]}
}

\newcommandx{\hproj}[2][1=\aH, 2=\ptp, usedefault=@]{
  \ifempty{#1}{}{{#1}}\ifempty{#2}{}{{^{\scriptscriptstyle @{#2}}}}
}
\newcommandx{\eproj}[2][1=\aE,2=A, usedefault=@]{
  {{#1}}\ifempty{#2}{}{{^{\scriptscriptstyle @{{\ptp[#2]}}}}}
}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%                        END CHOR MACROS                                %%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\apom}{r}
\newcommand{\emptypom}{\epsilon}
\newcommand{\emptyev}{\epsilon}
\newcommand{\alf}{\lambda}
\newcommand{\projpom}[2]{{#1}\!\!\downharpoonright_{#2}}
\newcommandx{\pomsetrep}[4][2=\alf, 3={}, 4={}, usedefault=@]{
  \left[
    \begin{array}[c]{c}
      \begin{tikzpicture}[every node/.style={pomset},#4]
        {#1;}
      \end{tikzpicture}
    \end{array}\right]_{#2}^{#3}
}
\tikzset{
  pomset/.style={
    scale = .7,
    transform shape,
    smooth
  }
}
\usetikzlibrary{lindenmayersystems}
\newcommand{\evconflict}[2]{\path[dashed] (#1) edge node[above]{\conflict} (#2);}
\newcommand{\evleq}[2]{\path[draw,->] (#1) -- (#2);}
\newcommand{\evstr}[2][.5]{
  \begin{tikzpicture}[node distance = #1 cm and #1 cm, every
	 node/.style={evstr}, transform shape]
	 {#2}
	 ;
  \end{tikzpicture}
}
\tikzset{
  evstr/.style={
    scale = .7,
    transform shape,
    smooth
  }
}

%%% chosem macros to add to ggmacros
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%                        START CHOSEM MACROS                            %%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\eset}{\mathcal{E}}
\newcommand{\aR}[1][R]{{\colorR{#1}}}
\newcommand{\efst}[1]{\pi_1\ifempty{#1}{}{({#1})}}
\newcommand{\aConf}{s}
\newcommand{\alfof}[1]{\alf_{#1}}
\newcommand{\minev}[1]{\mathtt{min}_{[#1]}}
\newcommand{\esetof}[1]{\eset_{#1}}
\newcommand{\leqof}[1]{\leq_{#1}}
\newcommandx{\detM}[1][1=\aCM,usedefault=@]{\Delta({#1})}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
%%%                        END CHOSEM MACROS                              %%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%                            CFSM MACROS                                %%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\alice}{\ptp[a]}
\newcommand{\carol}{\ptp[c]}
\newcommand{\bob}{\ptp[b]}
\newcommand{\dave}{\ptp[d]}
\newcommand{\msgfree}{\msg[free]}
\newcommand{\msgrequest}{\msg[sig]}
\newcommand{\msgscore}{\msg[score]}
\newcommand{\msgbusy}{\msg[busy]}
\newcommand{\msgcnowin}{\msg[close]}
\newcommand{\msgbnowin}{\msg[blose]}
\newcommand{\msgbwin}{\msg[bwin]}
\newcommand{\msgcwin}{\msg[cwin]}
\newcommand{\scenarioglobal}[1][.5]{
  \begin{tikzpicture}[node distance=0.43cm and 0.1cm,scale={#1},
    every node/.style={transform shape}]
    \node[source] at (0,0) (src) {};
    \node[agate, below=of src] (toppar) {};
    \node[ogate, below left= of toppar,xshift=-1cm] (topchoice) {};
    \node[block, below left=of topchoice] (b1) {$\gint[][\alice][\msgcwin][\carol]$};
    \node[block, below=of b1]  (b2) {$\gint[][\carol][\msgbnowin][\bob]$};
    \node[block, below right=of topchoice] (a1) {$\gint[][\alice][\msgbwin][\bob]$};
    \node[block, below=of a1] (a2) {$\gint[][\bob][\msgcnowin][\carol]$};
    \node[block, below right= of toppar,xshift=1cm] (c) {$\gint[][\carol][\msgbusy][\dave]$};
    \node[ogate, below=of b2]  (botchoice) at (b2-|topchoice) {};
    \node[agate, below=of botchoice]  (parsync) {};
    \node[block, below left=of parsync,yshift=-0.7cm] (d) {$\gint[][\bob][\msgrequest][\alice]$};
    \node[agate, below=of parsync] (botpar) at (parsync-|toppar) {};
    \node[block,below of= botpar] (e) at (d-|botpar) {$\gint[][\alice][\msgscore][\carol]$};
    \path [line] (src) -- (toppar);
    \path [line] (toppar) -| (topchoice);
    \path [line] (toppar) -| (c);
    \path [line] (c) |- (botpar);
    \path [line] (topchoice) -| (b1);
    \path [line] (topchoice) -| (a1);
    \path [line] (a1) -- (a2);
    \path [line] (b1) -- (b2);
    \path [line] (b2) |- (botchoice);
    \path [line] (a2) |- (botchoice);
    \path [line] (botchoice) -- (parsync);
    \path [line] (parsync) -| (d);
    \path [line] (parsync) -| (botpar);
    \path [line] (botpar) -- (e);
  \end{tikzpicture}
}

\newcommand{\cempty}{\mathbf{[]}}
\newcommandx{\cm}[2][1=\ptp, 2=\aM]{{#2}_{#1}}
% \newcommandx{\achan}[2][1=A,2=B,usedefault=@]{\overset{\to}{\ptp[{#1}]\,\ptp[{#2}]}}
\newcommandx{\achan}[2][1=A,2=B,usedefault=@]{{\ptp[#1]\,\ptp[#2]}}
\newcommand{\ptpset}{\mathcal{\colorPtp{P}}}
\newcommand{\PSet}{\ptpset}
\newcommand{\pset}{\ptpset}
\newcommand{\chan}[1]{\ptp[#1]}
\newcommand{\ASigma}{\msgset}
\newcommand{\oact}{\outop[]}
\newcommand{\iact}{\inop[]}
\newcommand{\tset}{\to}
\newcommand{\Smv}{\vec{S}}
\newcommand{\csconf}[2]{\conf{\vec{#1} \ ; \ \vec{#2}}}
\newcommand{\chanset}{\chset}
\newcommand{\TRANSS}[1]{{\xRightarrow{\raisebox{-.3ex}[0pt][0pt]{$\scriptstyle #1$} }}}
\newcommand{\RS}[1][]{\mathsf{RC}_{#1}}
\newcommand{\NUL}{\boldsymbol{}\varepsilon}
\newcommand{\asend}[3]{\ptp{#1} \! \rightarrowtriangle \! \ptp{#2} \!:\! \mbox{$\ptp{#3}$}}
\newcommand{\chosyn}{\chorgram}
\newcommand{\trans}[2][{}]{\,\xrightarrow{#2}_{#1}\,}
\newcommand{\cint}{\gint[{}]}
\newcommand{\cfsmTS}[1][0]{\mathit{TS}_{#1}}
\newcommandx{\acfsmout}[3][1=A,2=B,3=m,usedefault=@]{\achan[{#1}][{#2}] \oact {\msg[{#3}]}}
\newcommandx{\acfsmin}[3][1=A,2=B,3=m,usedefault=@]{\achan[{#1}][{#2}] \iact {\msg[{#3}]}}
\newcommandx{\fsaout}[2][1={\p},2={},usedefault=@]{
  \ptp[#1] \ \outop[]\ \msg[{#2}]
}
\newcommandx{\fsain}[2][1={\p},2={},usedefault=@]{
  \ptp[#1] \ \inop[]\ \msg[{#2}]
}

\makeatletter
\newcommand{\linenumfontsize}{\@setfontsize{\linenumfontsize}{3pt}{3pt}}
\makeatother
\lstset{
  numbers=left,
  numberstyle=\linenumfontsize,
  backgroundcolor=\color{black!3},
  basicstyle=\sffamily\tiny,
  tabsize=3,
  mathescape=true,
  morekeywords={of,do,system,||},
  morecomment=[l]{..},
  morecomment=[s]{[}{]},
  commentstyle=\color{blue!80!red!40},
  literate=*{=}{{\colorOp}{=}}{1}{||}{{\colorOp{||}}}{1}{+}{{\colorOp{+}}}{1}{!}{{\colorOpForestGreen}{!}}{1}{?}{{\colorOp{?}}}{1}{;}{{\colorOp{;}}}{1},
  keywordstyle=\color{ForestGreen}
 }

\lstdefinelanguage{sys}{
	commentstyle=\color{Gray},
%	morecomment=[l]{..},
	morecomment=[s]{[}{]},
   % keywordsprefix={receive},
	keywords=[0]{system,of,do,end},	keywordstyle=\color{orange}\bfseries,
%	morekeywords=[1]{\*,\+,\!,\?,\|,\=},	keywordstyle=[1]\color{blue}\bfseries,
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%                        END CFSM MACROS                                %%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%                          GRAPHS MACROS                                %%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\aG}{\mathsf{G}}
\newcommand{\gsink}{\circledcirc}
\newcommand{\gsource}{\circ}
\newcommand{\gvertex}{\bullet}
\newcommand{\gseqop}{{\colorOp ;}\,}
\newcommand{\gparop}{{\colorOp \ |\ }}
\newcommand{\gchoop}{{\colorOp \ +\ }}
\newcommand{\grecop}{{\colorOp *}}
\newcommand{\grecopp}{{\colorOp{@}}}
\newcommand{\gname}[1][i]{\ifcp{\colorNode{\scriptstyle\textsf{#1}}}{}\fi}
\newcommandx{\nmerge}[2][1={i},2={},usedefault=@]{
  \ifempty{#2}{
    \ifempty{#1}{\mu}{-\gname[{#1}]}
  }{-{#2}}
}

% \newcommand{\esbj}[1][\ae]{{\colorFun{\textsf{sbj}\ifempty{#1}{}{(#1)}}}}
\mkfun{\esbj}{sbj}{\ae}
\newcommand{\esubject}{\esbj}
\makeatletter%
\@ifclassloaded{exam-paper}%
  {}%
  {\makeatletter%
    \@ifclassloaded{test}%
    {}%
%    {\newcommand{\subject}{\esbj}}%
    \makeatother%
  }
\makeatother%


\newcommandx{\gnode}[2][1=\gname,2=\gint,usedefault=@]{
  {\ifempty{#1}{}{\colorNode{\gname[{#1}].}}} {#2}
}
\newcommand{\cpset}{\mathbb{\colorNode{Z}}_0}
\newcommand{\nodeset}{\cpset}
\newcommand{\gempty}{\mathbf{0}}
%\newcommandx{\gint}[4][1=,2=A,3=\msg,4=B,usedefault=@]{
%  \ptp[#2] {\colorOp \xrightarrow{ {\scriptscriptstyle\gname[#1]}{\hspace{.75em}} }} \ptp[#4] \colon {\msg[{#3}]}
%}
\newcommandx{\gint}[4][1=,2=A,3=\msg,4=B,usedefault=@]{
  \ptp[#2] {\colorOp \xrightarrow{\msg[{#3}]}} \ptp[#4]
}

\newcommand{\listptps}[1]{
  \def\ni{\def\nextitem{#1}}\@for \el:=.\do{\ptp[\ni].}
}
%\newcommandx{\refgint}[3][1=A,2=B,3=\msg,usedefault=@]{
%  \ptp[#1] {\colorOp \dashrightarrow} {
%    \renewcommand{\do}[1]{\ptp[##1]\ }
%    \docsvlist{#2}
%  }
%  \colon {\msg[{#3}]}
%}
\newcommandx{\refgint}[3][1=A,2=\msg,3=B,usedefault=@]{
  \ptp[#1] {\colorOp \xdashrightarrow[{}]{\msg[{#2}]}}{
    \renewcommand{\do}[1]{\ptp[##1]}
	 \docsvlist{#3}
  }
}
\newcommandx{\gout}[4][1=,2=\ptp,3=\msg,4={\ptp[C]},usedefault=@]{
  \achan[{#2}][{#4}] {\colorOp {\colorOp{!}}} {\msg[{#3}]}
}
\newcommandx{\gin}[4][1=,2=\ptp,3=\msg,4={\ptp[C]},usedefault=@]{
  \achan[{#2}][{#4}] {\colorOp {\colorOp{?}}} {\msg[{#3}]}
}
\newcommandx{\gseq}[3][1=,2={\aG},3={\aG'},usedefault=@]{
  \gnode[{#1}][{#2} \gseqop {#3}]
}
\newcommandx{\gpar}[3][1=,2={\aG},3={\aG'},usedefault=@]{
  \gnode[{#1}][\ifempty{#1}{{#2} \gparop {#3}}{({#2} \gparop {#3})}]
}
\newcommandx{\gcho}[3][1=,2={\aG},3={\aG'},usedefault=@]{
  \gnode[{#1}][\ifempty{#1}{{#2} \gchoop {#3}}{\big({#2} \gchoop {#3}\big)}]
}
\newcommandx{\gchov}[3][1=,2={\aG},3={\aG'},usedefault=@]{
  \gnode[{#1}][\left(
  \begin{array}l
    \ifempty{#1}{{#2} \\ \gchoop \\ {#3}}{\!\!{#2} \\ \gchoop \\ {#3}}
  \end{array}\right)
  ]
}
\newcommandx{\grec}[3][1=,2={\aG},3={\p},usedefault=@]{
  \gnode[{#1}][\ifempty{#1}{\grecop {#2} \grecopp {#3}}{\big(\grecop {#2} \grecopp {#3}\big)}]
}

\newcommand{\getcentroid}[2]{
    \coordinate (tmpgatecoord) at (0,0);
    \foreach \n [count=\i] in {#1}{
      \path (\n);
      \coordinate (tmpgatecoord) at ($(tmpgatecoord) + (\n)$);
      \coordinate (#2) at ($1/\i*(tmpgatecoord)$);
      %\node at (#2) {#2};
    }
}


\tikzset{
  hgsem/.style={
    draw,
    node distance=2cm and 1cm,
    transform shape,
    smooth,
    every node/.style = {font=\sffamily\bfseries}
  }
}

\tikzset{
  hgstyle/.style={
    src color={#1},
    tgt color={#1},
    centroid color={#1},
    centroid label={#1},
    centroid name={#1},
    centroid radius={#1},
    centroid ratio={#1},
    xoffset={#1},
    yoffset={#1},
    xsrcoffset={#1},
    ysrcoffset={#1},
    xtgtoffset={#1},
    ytgtoffset={#1},
    font={#1},
    centroid angle={#1},
    centroid tolerance={#1}
  },
  %
  src color/.store in = \hgsrccol,
  tgt color/.store in = \hgtgtcol,
  centroid color/.store in =\hgfillcolor,
  centroid label/.store in =\hglabel,
  centroid name/.store in =\hgname,
  centroid radius/.store in = \hgradius,
  centroid ratio/.store in = \hgratio,
  xoffset/.store in =\hgxoffset,
  yoffset/.store in =\hgyoffset,
  xsrcoffset/.store in =\hgxsrcoffset,
  ysrcoffset/.store in =\hgysrcoffset,
  xtgtoffset/.store in =\hgxtgtoffset,
  ytgtoffset/.store in =\hgytgtoffset,
  centroid angle/.store in =\hgangle,
  centroid tolerance/.store in =\hgtolerance,
  % 
  src color = black,
  tgt color = black,
  centroid color = orange!40,
  centroid label={},
  centroid name={dummycentroid},
  centroid radius = .7pt,
  centroid ratio = .35,
  xoffset = 0,
  yoffset = 0,
  xsrcoffset = 0,
  ysrcoffset = 0,
  xtgtoffset = 0,
  ytgtoffset = 0,
  font=\sffamily\scriptsize,
  centroid angle=0,
  centroid tolerance=10pt
}

\newcommandx{\mkhg}[5][1={},4={},5={},usedefault=@]{
  \begingroup
  \tikzset{#1}
  \StrCount{#2,}{,}[\l] % from package xxstring
  \StrCount{#3,}{,}[\m] % from package xxstring
  \ifthenelse{\l = 1 \AND \m = 1}{
    \ifempty{#4}{
      \ifempty{#5}{
        \path[hgsem, ->, >=stealth', shorten >=1pt] (#2) -- (#3);
      }{
        \path[hgsem, ->, >=stealth', shorten >=1pt] (#2) #5 (#3);
      }
    }{
      \ifempty{#5}{
        \path[hgsem, ->, >=stealth', shorten >=1pt, #4] (#2) -- (#3);
      }{
        \path[hgsem, ->, >=stealth', shorten >=1pt, #4] (#2) #5 (#3);
      }
    }
  }{
    \coordinate (srcoffset) at (\hgxsrcoffset,\hgysrcoffset);
    \coordinate (tgtoffset) at (\hgxtgtoffset,\hgytgtoffset);
    \getcentroid{#2}{srccentroid};
    \getcentroid{#3}{tgtcentroid};
    \node[label={left:\hglabel}] (\hgname) at ($(srccentroid)!{1-\hgratio}!\hgangle:(tgtcentroid) + (\hgxoffset,\hgyoffset)$) {};
    \pgfgetlastxy \xc \yc;
    \pgfmathtruncatemacro{\xcontrol}{\xc};
    \pgfmathtruncatemacro{\ycontrol}{\yc};
    \foreach \n in {#2}{
      \path (\n);
      \pgfgetlastxy \xntmp \yntmp;
      \pgfmathtruncatemacro{\xn}{\xntmp};
      \pgfmathtruncatemacro{\yn}{\yntmp};
      \pgfmathsetmacro\xtmpdiff{abs(\xn - \xcontrol + \hgxsrcoffset)};
      \pgfmathsetmacro\ytmpdiff{abs(\yn - \ycontrol + \hgytgtoffset)};
      \ifdim \xtmpdiff pt > \hgtolerance
      \ifempty{#4}{
        \path[hgsem, \hgsrccol] (\n) .. controls ($(srccentroid.center) + (srcoffset)$) .. (\hgname.center);
      }{
        \path[hgsem, \hgsrccol] (\n) .. controls ($(srccentroid.center) + (srcoffset)$) .. (\hgname.center);
      }
      \else
      \ifempty{#4}{
        \path[hgsem, \hgsrccol] (\n) -- (\hgname.center);
      }{
        \path[hgsem, \hgsrccol, #4] (\n) -- (\hgname.center);
      }
      \fi
    }
    \foreach \n in {#3}{
      \path (\n);
      \pgfgetlastxy \xntmp \yntmp;
      \pgfmathtruncatemacro{\xn}{\xntmp};
      \pgfmathtruncatemacro{\yn}{\yntmp};
      \pgfmathsetmacro\xtmpdiff{abs(\xn - \xcontrol)};
      \pgfmathsetmacro\ytmpdiff{abs(\yn - \ycontrol)};
      \ifdim \xtmpdiff pt > \hgtolerance
      \ifempty{#4}{
        \path[hgsem, ->, >=stealth', shorten >=1pt, \hgtgtcol] (\hgname.center) .. controls (tgtcentroid.center) and ($(tgtcentroid.center) + (tgtoffset)$) .. (\n);
      }{
        \path[hgsem, ->, >=stealth', shorten >=1pt, \hgtgtcol,#4] (\hgname.center) .. controls (tgtcentroid.center) and ($(tgtcentroid.center) + (tgtoffset)$) .. (\n);
      }
      \else
      \ifempty{#4}{
        \path[hgsem, ->, >=stealth', shorten >=1pt, \hgtgtcol] (\hgname.center) --  (\n);
      }{
        \path[hgsem, ->, >=stealth', shorten >=1pt, \hgtgtcol] (\hgname.center) --  (\n);
      }
      \fi
    }
    \fill[\hgfillcolor] (\hgname) circle [radius=\hgradius];
  }
  \endgroup
}

\newcommand{\hghb}[1]{\widehat{#1}}
\newcommandx{\hgordeq}[1][1={\aH},usedefault=@]{\sqsubseteq_{#1}}
%
\newcommandx{\gintsem}[4][4=.5]{
  \tikz[hgsem,scale=#4,every node/.style={font=\scriptsize}]{
    \node (out) {$\aout[{#1}][{#2}][][{\msg[{#3}]}]$};
    \node[below = 20pt of out] (in) {$\ain[{#1}][{#2}][][{\msg[{#3}]}]$};
    \mkhg{out}{in};
  }
}

\newcommandx{\gsem}[2][1={\aG},2={},usedefault=@]{[\![ {#1} ]\!]_{#2}}
\newcommandx{\rbot}{\text{undef}}
\newcommandx{\rtrs}[1][1={\aH},usedefault=@]{{#1}^{\star}}
\newcommandx{\gord}[1][1={\aG},usedefault=@]{\leq_{#1}}
\newcommandx{\gordeq}[1][1={\aG},usedefault=@]{\leq_{#1}}
\mkfun{\cause}{cs}{}
\mkfun{\effect}{ef}{}
% \newcommandx{\efst}[1]{\textsf{cs}\ifempty{#1}{}{_{({#1})}}}
\newcommand{\hgflattening}[1]{\widehat{#1}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%                      END GRAPHS MACROS                                %%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%to remove
\newcommandx{\aW}{w}
\newcommandx{\rlang}{\mathcal{L}}
%\newcommand{\enode}[1]{{\colorAct{\textsf{cp}}\ifempty{#1}{}{({#1})}}}
% \newcommand{\eact}[1]{{\colorAct{\textsf{act}}}\ifempty{#1}{}{({#1})}}
\newcommand{\gfun}[1]{\ensuremath{\mathsf{\colorFun #1}}}
\mkfun{\eact}{\gfun{act}}{}
\mkfun{\enode}{\gfun{cp}}{}

\mkuop{\rmax}{\gfun{max}}{\aH}
\mkuop{\rmin}{\gfun{min}}{\aH}
\mkuop{\rMAX}{\gfun{lst}}{\aH}
\mkuop{\rMIN}{\gfun{fst}}{\aH}
\newcommand{\rlt}[1][\aH]{<_{#1}}
\newcommandx{\rseq}[2][1=\aG,2={\aG'},usedefault=@]{\gfun{seq}({#1},{#2})}
\newcommandx{\rpar}[2][1=\aG,2={\aG'},usedefault=@]{\gfun{par}({#1},{#2})}

\newcommandx{\gproj}[2][1=\aG,2=\ptp]{{#1}\downarrow_{#2}}
\newcommandx{\cinit}[1][1={\aQzero},usedefault=@]{{#1}}
\newcommandx{\cfinal}[1][1={q_e},usedefault=@]{{#1}}
\newcommand{\ctr}[3]{
  \tikz{
    \node at (0,0) (i) {};
    \node[shape=circle,draw,inner sep=1pt] at (0.6,0) (s) {$#1$};
    \node[shape=circle,draw,inner sep=1pt, right=of s] at (1.7,0)  (t) {$#2$};
    \node at (3.2,0) (f) {};
    \draw[->] (i) -- (s);
    \draw[->] (s) -- (t) node [midway,above]{$#3$};
    \draw[->] (t) -- (f);
  }
}
\newcommand{\ccup}{\sqcup}
\newcommand{\ccap}{\cap}
\newcommand{\cprod}{\otimes}
\newcommandx{\geproj}[4][1=\aG,2=\ptp,3=\cinit,4=\cfinal,usedefault=@]{
  {#1}\downarrow_{#2}^{{#3},{#4}}
}

\newcommand*{\StrikeThruDistance}{0.15cm}%
\newcommand*{\StrikeThru}{\StrikeThruDistance,\StrikeThruDistance}%
\tikzset{strike thru arrow/.style={
    decoration={markings, mark=at position 0.5 with {
        \draw [blue, thick,-] 
            ++ (-\StrikeThruDistance,-\StrikeThruDistance) 
            -- ( \StrikeThruDistance, \StrikeThruDistance);}
    },
    postaction={decorate},
}}


\newcommandx{\ich}[1][1={\aG},usedefault=@]{{#1}^{\oplus}}
\newcommandx{\ichedges}[2][1={\aG},2={\gname},usedefault=@]{{#1}^{\oplus}({#2})}
\newcommandx{\parts}[1]{2^{#1}}
\newcommandx{\actch}{c}
\newcommandx{\soundactch}[2][1={\aG},2={\actch},usedefault=@]{{#1} \,\circledR\, {#2}}
\newcommandx{\rOnActch}[2][1={\aG},2={\actch},usedefault=@]{{#1} \setminus {#2}}
\newcommandx{\rOnActchClean}[2][1={\aG},2={\actch},usedefault=@]{{#1} \circledR {#2}}
\newcommandx{\rAllEvents}[1][1={\aG},usedefault=@]{\mathit{dom}(#1)}

\newcommand{\av}{\ae}
\newcommand{\aV}{\aE}
\newcommand{\AV}{\mathcal{V}}
\newcommand{\aH}{H}
\newcommand{\ah}{h}
\newcommandx{\hgvertex}[2][1=\al,2=\gname,usedefault=@]{{#1}_{\textcolor{red}{[{#2}]}}}
\newcommand{\aE}{{\colorE E}}
\renewcommand{\ae}[1][e]{{\colorE{#1}}}
\newcommand{\aL}{{\tilde \al}}
\newcommand{\al}[1][l]{{\colorE{#1}}}
\newcommandx{\hyedge}[1]{\{#1\}}

\newcommandx{\rdiv}[2][1=\gcho,2=\ptp,usedefault=@]{
  \gfun{div}_{#2}(#1)
}

\newcommandx{\rrdiv}[5][1={\aG},2={\aG'},3={\AV},4={\AV'},5=\ptp,usedefault=@]{
  \gfun{div}^{#3,#4}_{#5}(#1,#2)
%#1 \xhookleftarrow{#3} \!\!{_{#5}} \!\!\xhookrightarrow{#4} #2
}
\newcommandx{\pdiv}[3][1={\apom_1},2={\apom_2},3={\apom},usedefault=@]{
  \gfun{div}_{#3}(#1,#2)
%#1 \xhookleftarrow{#3} \!\!{_{#5}} \!\!\xhookrightarrow{#4} #2
}
\newcommandx{\pfork}[3][1={\apom_1},2={\apom_2},3={\apom},usedefault=@]{
  \gfun{fork}_{#3}(#1,#2)
%#1 \xhookleftarrow{#3} \!\!{_{#5}} \!\!\xhookrightarrow{#4} #2
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%                            TIKZ MACROS                                %%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\newcommandx{\mkint}[6][3=i,4=\p,5=\msg,6=\q,usedefault=@]{
%  \node[bblock\ifempty{#1}{}{,{#1}}] \ifempty{#1}{at (0,0)}{} (#2) {$\gint[#3][#4][#5][#6]$};
  \node[bblock, #1] (#2) {$\gint[#3][#4][#5][#6]$};
}

\newcommand{\mkseq}[2]{\path[line] (#1) -- (#2);}

\newcommand{\mknseq}[1]{
  \StrCount{#1}{,}[\l] % from package xxstring
  \StrBefore{#1}{,}[\myhead]
  \StrBehind{#1}{,}[\mytail]
  \StrBefore{\mytail}{,}[\sndel]
  \ifnum \l > 1 {
    \mkseq{\myhead}{\sndel};
    \mknseq{\mytail}
  }
  \else{\ifnum \l > 0{
      \mkseq{\myhead}{\mytail};
    }
    \else{}
    \fi
  }
  \fi
}

\newcommandx{\mkgateblock}[6][6=yellow!10,usedefault=@]{
  % #1: gate
  % #2: position of opening gate
  % #3: comma-separated list of children of opening gate
  % #4: comma-separated list of parents of closing gate
  % #5: position of closing gate
  % #6: background color
  \path(#2);
  \pgfgetlastxy{\xgate}{\ygate};
  \pgfmathtruncatemacro{\xgateround}{\xgate};
  \StrCount{#3,}{,}[\l] % from package xstring
  \ifnum \l < 2 {\errmessage{#3 argument should be a comma-separated list of lenght >= 2}}
  \else{
    \foreach \n in {#3}{
      \path (\n);
      \pgfgetlastxy{\xnode}{\ynode};
      \pgfmathtruncatemacro{\xnround}{\xnode};
      \pgfmathsetmacro\tmpdiff{abs(\xnround - \xgateround)}
      \ifdim \tmpdiff pt > 1 pt \path[line] (#2) -| (\n);
      \else
        \path[line] (#2) -- (\n);
      \fi
    }
  }
  \fi
  \StrCount{#4,}{,}[\l] % from package xstring
  \ifnum \l < 2 {\errmessage{#4 argument should be a comma-separated list of lenght >= 2}}
  \else{
    \foreach \n in {#4}{
      \path (\n);
      \pgfgetlastxy{\xnode}{\ynode};
      \pgfmathtruncatemacro{\xnround}{\xnode};
      \pgfmathsetmacro\tmpdiff{abs(\xnround - \xgateround)}
      \ifdim \tmpdiff pt > 1 pt \path[line] (\n) |- (#5);
      \else
        \path[line] (\n) -- (#5);
      \fi
    }
  }
  \fi
  \node[#1] at (#2) {};
  \node[#1] at (#5) {};
  {
    \begin{pgfonlayer}{background}
      \path[fill=#6,rounded corners]
      (current bounding box.south west) rectangle
      (current bounding box.north east);
    \end{pgfonlayer}
  }
}

\newcommandx{\mkbranchblock}[5][5=@]{
  \mkgateblock{ogate}{#1}{#2}{#3}{#4}[#5]
}

\newcommandx{\mkforkblock}[5][5=@]{
  \mkgateblock{agate}{#1}{#2}{#3}{#4}[#5]
}

\newcommandx{\mkgraph}[3][1=.5cm, usedefault=@]{
  \node[source,above = #1 of {#2}] (src#2) {};
  \node[sink,below  = #1 of {#3}] (sink#3) {};
  \path[line] (src#2) -- (#2);
  \path[line] (#3) -- (sink#3);
}

\newcommandx{\mkloop}[5][1=.5, 2=1.5, 5=\aguard, usedefault=@]{
  \node[lgate,above = #1 of {#3}] (entry#3) {};
  \pgfgetlastxy \xentry \yentry;
  \pgfmathtruncatemacro{\xentryrounded}{\xentry};
  \node[below = #1 of {#4}, label = {above right:{$#5$}},yshift=-1em] (dummy) {};
  \node[lgate,below  = #1 of {#4}] (exit#4) {};
  \pgfgetlastxy \xexit \yexit;
  \pgfmathtruncatemacro{\xexitrounded}{\xexit};
  \path[line] (entry#3) -- (#3);
  \path[line] (#4) -- (exit#4);
  \pgfmathsetmacro\tmpdiff{abs(\xentryrounded - \xexitrounded)}
  \path[line, color=teal] (exit#4) -| ($(exit#4)+(\tmpdiff,0)+(#2,0)$) |- (entry#3);
}

\newcommandx{\mkfork}[4][2=gatenode,3=i,4=.6,usedefault=@]{
  \mkgatebegin{#1}[{\gname[#3]}][agate][#4]{#2}
}

\newcommandx{\mkbranch}[4][2=gatenode,3=i,4=.6,usedefault=@]{
  \mkgatebegin{#1}[{\gname[#3]}][ogate][#4]{#2}
}

\newcommandx{\mkgatebegin}[5][2={},3=ogate,4=.5,usedefault=@]{
  % #1: list of nodes
  % #2: control point
  % #3: gate type
  % #4: vertical position offset
  % #5: name of the gate node
  %
  \coordinate (gatecord) at (0,0);
  \coordinate (xmax) at (0,0);
  \coordinate (xmin) at (0,0);
  \pgfgetlastxy \xmin \xmax;
  \foreach \n [count=\i] in {#1}{
    \pgfgetlastxy \xc \yc;
    \path (\n);
    \pgfgetlastxy \xn \yn;
    \ifnum \i = 1
      \coordinate (xmin) at (\xn,0);
      \coordinate (xmax) at (\xn,0);
      \coordinate (max) at (0,\yn);
    \else
      \ifdim \xn < \xmin
        \coordinate (xmin) at (\xn,0);
      \fi
      \ifdim \xn > \xmax
        \coordinate (xmax) at (\xn,0);
      \fi
      \ifdim \yn < \yc
        \coordinate (max) at (0,\yc);
      \else
        \coordinate (max) at (0,\yn);
      \fi
    \fi
  }
  \coordinate (gatecord) at ($(xmin)!.5!(xmax) + (max) + (0,#4) + (max)$);
  \node[#3,label={below:$#2$}] (#5) at (gatecord) {};
  \pgfgetlastxy{\xgate}{\ygate};
  \pgfmathtruncatemacro{\xgateround}{\xgate};
  \StrCount{#1,}{,}[\l] % from package xxstring
  \ifnum \l < 2 {\errmessage{#1 argument should be a comma-separated list of lenght >= 2}}
  \else{
    \foreach \n in {#1}{
      \path (\n);
      \pgfgetlastxy{\xnode}{\ynode};
      \pgfmathtruncatemacro{\xnround}{\xnode};
      \pgfmathsetmacro\tmpdiff{abs(\xnround - \xgateround)}
      \ifdim \tmpdiff pt > 1 pt \path[line] (#5) -| (\n);
      \else
        \path[line] (#5) -- (\n);
      \fi
    }
  }
  \fi
}

\newcommandx{\mkgatebeginold}[5][2={},3=ogate,4=.5,usedefault=@]{
  % #1: list of nodes
  % #2: control point
  % #3: gate type
  % #4: vertical position offset
  % #5: name of the gate node
  %
  \coordinate (gatecord) at (0,0);
  \foreach \n [count=\i] in {#1}{
    \pgfgetlastxy \xc \yc;
    \path (\n);
    \pgfgetlastxy \xn \yn;
    \coordinate (gatecord) at ($(gatecord) + (\xn,0)$);
    \coordinate (gatecord) at ($1/\i*(gatecord)$);
    \ifdim \yn < \yc
    \node (max) at (0,\yc) {};
    \else
    \node (max) at (0,\yn) {};
    \fi
  }
  \coordinate (gatecord) at ($(gatecord) + (0,#4) + (max)$);
  \node[#3,label={below:$#2$}] (#5) at (gatecord) {};
  \pgfgetlastxy{\xgate}{\ygate};
  \pgfmathtruncatemacro{\xgateround}{\xgate};
  \StrCount{#1,}{,}[\l] % from package xxstring
  \ifnum \l < 2 {\errmessage{#1 argument should be a comma-separated list of lenght >= 2}}
  \else{
    \foreach \n in {#1}{
      \path (\n);
      \pgfgetlastxy{\xnode}{\ynode};
      \pgfmathtruncatemacro{\xnround}{\xnode};
      \pgfmathsetmacro\tmpdiff{abs(\xnround - \xgateround)}
      \ifdim \tmpdiff pt > 1 pt \path[line] (#5) -| (\n);
      \else
        \path[line] (#5) -- (\n);
      \fi
    }
  }
  \fi
}

\newcommandx{\mkmerge}[4][2=gatenode,3=i,4=.5,usedefault=@]{\mkgateend{#1}[{\ifempty{#3}{}{\nmerge[#3]}}][ogate][#4]{#2}}

\newcommandx{\mkjoin}[4][2=gatenode,3=i,4=.5,usedefault=@]{\mkgateend{#1}[{\ifempty{#3}{}{\nmerge[#3]}}][agate][#4]{#2}}

\newcommandx{\mkgateend}[5][2={},3=ogate,4=.5,usedefault=@]{
  % #1 list of nodes
  % #2 control point
  % #3 gate type
  % #4 vertical position offset
  % #5 name of the gate node
  %
  \coordinate (gatecord) at (0,0);
  \coordinate (xmax) at (0,0);
  \coordinate (xmin) at (0,0);
  \pgfgetlastxy \xmin \xmax;
  \foreach \n [count=\i] in {#1}{
    \pgfgetlastxy \xc \yc;
    \path (\n);
    \pgfgetlastxy \xn \yn;
    \ifnum \i = 1
      \coordinate (xmin) at (\xn,0);
      \coordinate (xmax) at (\xn,0);
      \coordinate (ymin) at (0,\yn);
    \else
      \ifdim \xn < \xmin
        \coordinate (xmin) at (\xn,0);
      \fi
      \ifdim \xn > \xmax
        \coordinate (xmax) at (\xn,0);
      \fi
      \ifdim \yn > \yc
        \coordinate (ymin) at (0,\yc);
      \else
        \coordinate (ymin) at (0,\yn);
      \fi
    \fi
  }
  \coordinate (gatecord) at ($(xmin)!.5!(xmax) + (ymin)$);
  \node[#3,label={above:$#2$}] (#5) at ($(gatecord) - (0,{#4})$) {};
  \pgfgetlastxy{\xgate}{\ygate};
  \pgfmathtruncatemacro{\xgateround}{\xgate};
  \StrCount{#1,}{,}[\l] % from package xstring
  \ifnum \l < 2 {\errmessage{#1 argument should be a comma-separated list of lenght >= 2}}
  \else{
    \foreach \n in {#1}{
      \path (\n);
      \pgfgetlastxy{\xnode}{\ynode};
      \pgfmathtruncatemacro{\xnround}{\xnode};
      \pgfmathsetmacro\tmpdiff{abs(\xnround - \xgateround)}
      \ifdim \tmpdiff pt > 1 pt \path[line] (\n) |- (#5);
      \else
        \path[line] (\n) -- (#5);
      \fi
    }
  }
  \fi
}

\newcommandx{\mkgateendold}[5][2={},3=ogate,4=.5,usedefault=@]{
  % #1 list of nodes
  % #2 control point
  % #3 gate type
  % #4 vertical position offset
  % #5 name of the gate node
  %
  \coordinate (gatecord) at (0,0);
  \coordinate (xmax) at (0,0);
  \coordinate (xmin) at (0,0);
  \pgfgetlastxy \xmin \xmax;
  \foreach \n [count=\i] in {#1}{
    \pgfgetlastxy \xc \yc;
    \path (\n);
    \pgfgetlastxy \xn \yn;
    \ifdim \xn < \xmin
    \coordinate (xmin) at (\xn,0);
    \fi
    \ifdim \xn > \xmax
    \coordinate (xmax) at (\xn,0);
    \fi
    \ifdim \yn > \yc
    \coordinate (ymin) at (0,\yc);
    \else
    \coordinate (ymin) at (0,\yn);
    \fi
    \coordinate (gatecord) at ($(xmin)!.5!(xmax) + (ymin)$);
  }
  \node[#3,label={above:$#2$}] (#5) at ($(gatecord) - (0,{#4})$) {};
  \pgfgetlastxy{\xgate}{\ygate};
  \pgfmathtruncatemacro{\xgateround}{\xgate};
  \StrCount{#1,}{,}[\l] % from package xstring
  \ifnum \l < 2 {\errmessage{#1 argument should be a comma-separated list of lenght >= 2}}
  \else{
    \foreach \n in {#1}{
      \path (\n);
      \pgfgetlastxy{\xnode}{\ynode};
      \pgfmathtruncatemacro{\xnround}{\xnode};
      \pgfmathsetmacro\tmpdiff{abs(\xnround - \xgateround)}
      \ifdim \tmpdiff pt > 1 pt \path[line] (\n) |- (#5);
      \else
        \path[line] (\n) -- (#5);
      \fi
    }
  }
  \fi
}


\newcommand{\ggateopen}[3][]{
  \ifempty{#1}{}{\path[line] (#1) -- (#2);}
  \foreach \x in {#3} \path[line] (#2) -| (\x);
}

\newcommand{\ggateclose}[3][]{
  \foreach \x in {#3} \path[line] (\x) |- (#2);
  \ifempty{#1}{}{\path[line] (#2) -- (#1);}
}

\newcommand{\gatedistancein}{3pt}
\newcommand{\gatedistanceinand}{2pt}

\usetikzlibrary{
  arrows,
  backgrounds,
  chains,
  calc,
  decorations.markings,decorations.pathreplacing,
  fadings,
  fit,
  patterns,
  petri,
  positioning,
  shadows,
  shapes,automata,shapes.callouts
}

\newcommand{\sourceG}{
  \begin{tikzpicture}[smallglobal,baseline=-.5ex, scale=0.6, every node/.style={transform shape}]
  \node [source] (src) {};
\end{tikzpicture}
}

\newcommand{\sinkG}{
\begin{tikzpicture}[smallglobal,baseline=-.5ex, scale=0.6, every node/.style={transform shape}]
  \node [sink] (src) {};
\end{tikzpicture}
}

\newcommand{\orgateG}{
\begin{tikzpicture}[smallglobal,baseline=-.5ex, scale=0.75, every node/.style={transform shape}]
  \node [ogate] (o) {};
\end{tikzpicture}
}

\newcommand{\lgateG}{
\begin{tikzpicture}[smallglobal,baseline=-.5ex, scale=0.75, every node/.style={transform shape}]
  \node [lgate] (o) {};
\end{tikzpicture}
}

\newcommand{\andgateG}{
\begin{tikzpicture}[smallglobal,baseline=-.5ex, scale=0.75, every node/.style={transform shape}]
  \node [agate] (o) {};
\end{tikzpicture}
}

\tikzset{
  src/.style={draw,circle,fill=white,
    minimum size=2mm,
    inner sep=0pt
  },
  sink/.style={draw,circle,double,fill=white,
    minimum size=1.5mm,
    inner sep=0pt
  },
  node/.style={draw,circle,fill=black,
    minimum size=2mm,
    inner sep=0pt
  },
  % 
  source/.style={draw,circle,fill=white,
    minimum size=3mm,
    inner sep=0pt
  },
  sink/.style={draw,circle,double,fill=white,
    minimum size=3mm,
    inner sep=0pt
  },
  % ACTION
  block/.style = {rectangle, draw=gray, align=center, fill=orange!25, rounded corners=0.1cm,
    minimum size=5mm, inner sep=2pt},
  prenode/.style = {minimum size=9pt,inner sep=2pt, font=\Large},
  % 
  bblock/.style = {rectangle, draw=blue!50, opacity=.7, line width=.5pt, align=center, fill=white, rounded corners=0.1cm,
    minimum size=4mm, inner sep=1pt},
  prenode/.style = {minimum size=9pt,inner sep=2pt, font=\Large},
  % AND GATE
  agate/.style={draw, rectangle,
    minimum size=3mm,
    inner sep=0pt,
    fill=orange!25,
    label={[red]center:$\mid$}
  },
  % ORGATE
  ogate/.style = {
    diamond, draw, fill=orange!25,
    minimum size=4mm,
    inner sep=0pt,
    label={[red]center:$+$}
  },
  % LOOP GATE
  lgate/.style = {
    diamond, draw, fill=orange!25,
    minimum size=4mm,
    inner sep=0pt,
    label={[red]center:$\circlearrowleft$}
    },
  % 
  altogate/.style = {
    diamond, draw,
    minimum size=4mm,
    inner sep=0pt,
    postaction={path picture={% 
        \draw
        ([yshift=\gatedistancein]path picture bounding box.south) -- ([yshift=-\gatedistancein]path picture bounding box.north)
        ([xshift=-\gatedistancein]path picture bounding box.east) -- ([xshift=\gatedistancein]path picture bounding box.west)
        ;}}},
  altgate/.style={draw, rectangle,
    minimum size=3mm,
    inner sep=0pt,
    postaction={path picture={% 
        \draw
        ([yshift=\gatedistanceinand]path picture bounding box.south) --
        ([yshift=-\gatedistanceinand]path picture bounding box.north) ;}}},
  % ogate or agate
  anygate/.style = {circle, draw, fill=white,
    minimum size=4mm,
    inner sep=0pt,
    postaction={path picture={% 
        \draw[black]
        ([xshift=-\gatedistancein,yshift=\gatedistancein]path picture bounding box.south east) --
        ([xshift=\gatedistancein,yshift=-\gatedistancein]path picture bounding box.north west)
        ([xshift=-\gatedistancein,yshift=-\gatedistancein]path picture bounding box.north east) --
        ([xshift=\gatedistancein,yshift=\gatedistancein]path picture bounding box.south west)
        ;}}
  },
  % 
  smallglobal/.style={
        node distance=1cm and 0.8cm, semithick, scale=0.8, every node/.style={transform shape}
  },
  % DOTS
  elli/.style = {draw,densely dotted,-},
  % 
  % LINES
  line/.style = {draw,->, rounded corners=0.07cm,>=latex},
  nline/.style = {draw,semithick, ->},
  pline/.style = {draw,->,>=latex},
  node distance=1cm and 0.7cm,
  baseline=(current  bounding  box.center),
  local/.style={rectangle, draw, fill=\fillcolor, drop shadow,
    text centered, rounded corners, minimum height=5em
  },
  bigar/.style={
    draw,very thick, ->
  },
  process/.style={rectangle, draw=gray, fill=\fillcolor, drop shadow,
    text centered, minimum height=5em,text=gray
  },
  choreo/.style={rectangle, draw, fill=\fillcolor, drop shadow,
    text centered, rounded corners, minimum height=5em
  },
  % CFSM
  mycfsm/.style={
        font=\footnotesize,
        initial where=above,
        ->,>=stealth,auto, node distance=1cm and 1cm,
        scale=1, every node/.style={transform shape},
        every state/.style=inner sep=2pt,
        baseline=(current  bounding  box.center),
        initial text={}
  },
  machinecloud/.style={
    cloud, cloud puffs=10, cloud ignores aspect, minimum height=.1cm, minimum width=2cm, draw
  },
  fitting node/.style={
    inner sep=0pt,
    fill=none,
    draw=none,
    reset transform,
    fit={(\pgf@pathminx,\pgf@pathminy) (\pgf@pathmaxx,\pgf@pathmaxy)}
  },
  mypetri/.style={
    font=\footnotesize,
    baseline=(current  bounding  box.center)
  },
  silentrans/.style = {rectangle, draw=black, align=center, fill=black,
    minimum height=1pt,
    minimum width=15pt,
    inner sep=1.5pt
  },
  reset transform/.code={\pgftransformreset},
  tmtape/.style={draw,minimum size=1.2cm}
}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%                        END TIKZ MACROS                                %%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\newcommand{\gtryop}{{\colorOp try}}
\newcommand{\gdoop}{{\colorOp do}}
\newcommand{\gunlessop}{\mbox{\colorOp\tiny\tt unless}}
\newcommand{\gwithop}{{\colorOp with}}
\newcommand{\gcatchop}{{\colorOp catch}}
\newcommand{\gonop}{{\colorOp on}}

\newcommandx{\gtry}[5][1=\gname,2={\aG_1 \gchoop \cdots \gchoop \aG_n},3=\gin,4=\gout,5={j},usedefault=@]{
  \def\foo{\gtryop\ {#2} \ \gcatchop\ {#3} {\colorOp \Rightarrow} {#4} {\colorOp \bullet} {\gname[{#5}]}}
  \gnode[{#1}][{\ifempty{#1} {\foo } { \big(\foo \big) }}]
}

\newcommandx{\gtrycatch}[4][1=\gname,2={\aG},3=\gin,4={\aG'},usedefault=@]{
  \def\foo{\gtryop\ {#2} \ \gcatchop\ {#3} \gdoop\ {#4}}
  \gnode[{#1}][{\ifempty{#1} {\foo} {\big( \foo \big) }}]
}

\def\colorGuard{\color{cyan}}
\newcommand{\aguard}{{\colorGuard \phi}}
\newcommandx{\agG}[2][1={\aG},2=\aguard]{{#1} \ifempty{#2}{}{\ \gunlessop\ {#2}}}

\newcommandx{\grcho}[5][1=\gname,2={\agG},3={\agG[\aG'][\aguard']},4={\cdots},5=A,usedefault=@]{
  \def\foo{{#2} {\ \ifempty{#4}{\gchoop}{\gchoop \ifempty{#4}{}{\ {#4}\  \gchoop}}\ } {#3}}
  \ifempty{#1}{\ifempty{#5}{\foo}{\gselop\ \cpt[{#1}][{\ptp[#5]}]\big\{ \foo \big\}}}{\gselop\ \cpt[{#1}][{\ptp[#5]}]\big\{ \foo \big\}}
}

\newcommandx{\ggprefix}[3][1=\ptp,2={\aR},3={\aR'},usedefault=@]{f_{#1}} % it was \newcommandx{\common}{...}
\newcommand{\aconfigfn}{\chi}
\newcommand{\aconfig}{\ell}
\newcommand{\aqueue}[2]{{#1}\ ;\ {#2}}
\newcommand{\lstates}{\statemap}
\newcommandx{\sysconfig}[3][1=\lstates,2=\aconfigfn,3={},usedefault=@]{
  \conf{ {#1},{#2} \ifempty{#3}{}{, #3} }
}
\newcommand{\sysctxfn}[1][]{\gamma_{#1}}
\newcommandx{\sysctx}[2][1=\aQ,2={},usedefault=@]{({#1},\sysctxfn[{#2}])}
\newcommand{\natnums}{\mathbb{N}}
\newcommand{\apred}[1][p]{\mathtt{#1}}
\newcommand{\eventof}[1][\gname]{\mathsf{event}(\ifempty{#1}{\_}{#1}) }
\newcommand{\logset}{\mathsf{Log}}
\newcommand{\comsysQ}[1][]{\mathcal{\aQ}_{#1}}
\newcommandx{\alog}[4][1=\msg,2=q,3=\gname,4=t,usedefault=@]{\big({#1},{#2},{#3},{#4}\big)}
\newcommand{\cfsmQ}[1][\p]{{\aQ_{#1}}}
\newcommand{\aCM}{M}\newcommand{\aM}{\aCM}
\newcommand{\aQ}{Q}
\newcommandx{\aQzero}[1][1=,usedefault=@]{
  {\ifempty{#1}{q_0}{q_{0#1}}}
}
\newcommand{\badbranches}[1][]{\beta\ifempty{#1}{}{\big({#1}\big)}}
\newcommand{\aTrs}{\tset}
\newcommandx{\guardedaction}[2][1=\al,2=\aguard,usedefault=@]{
  {#1} \ifempty{#2}{}{/} {#2}
}
\newcommandx{\atrM}[4][1=q,2=\al,3={\hat q,\hat \al, \aguard},4=q',usedefault=@]{
  {#1} \xrightarrow[{#3}]{\guardedaction[{#2}][]} {{#4}}
}
\newcommandx{\atrS}[5][
  1={\sysconfig[@][@][\badbranches]},
  2=\al,
  3=\aguard,
  4={\sysconfig[\lstates'][\aconfigfn'][\badbranches]},
  5=\sysctx,usedefault=@
]{
  {#1} \xRightarrow{\qquad} {{#4}}
}
\newcommandx{\arevtrS}[2][
  1={\sysconfig[@][@][\badbranches]},
  2={\sysconfig[\lstates'][\aconfigfn'][\badbranches']},
  usedefault=@
]{
  {#1} \rightsquigarrow {#2}
}
\newcommand{\aCS}{S}
\newcommand{\abuffer}{b}
\newcommand{\guardset}{{\Phi}}
\newcommandx{\enables}[2][1=\aconfigfn,2=\aguard,usedefault=@]{{#1} \vdash {#2}}
\newcommandx{\gprojfn}[5][1=\aG,2=\ptp,3=\cinit,4=\cfinal,5={},usedefault=@]{
  \mathbf{proj}_{#2}({#1},{#3},{#4}\ifempty{#5}{}{,{#5}})
}

\newcommandx{\rbp}[3][1=\aG,2=\aconfigfn,3=\achan,usedefault=@]{\mathtt{RBP}_{{#1},{#2}}\ifempty{#3}{}{\big({#3}\big)}}

\newcommand{\apseudoCFSM}{\mathtt{M}}
\newcommandx{\pseudoseq}[2][1=\apseudoCFSM,2=\apseudoCFSM',usedefault=@]{{#1}  ; {#2}}
\newcommandx{\pseudoCFSM}[4][1=\aQ,2=\aQzero,3=\cfinal,4=\aTrs,usedefault=@]{(#1 \ ; #2 \ ; #3 \ ; #4)}
\newcommandx{\markt}[3][1=\hat{\al},2=\hat{q},3=\aguard,usedefault=@]{\%\big({#1} , {#2}, {#3}\big)}
\newcommand{\forget}[1][]{ \mathsf{forget}\ifempty{#1}{}{\big( {#1} \big)} }
\newcommand{\lift}[1][]{\mathsf{lift}\ifempty{#1}{}{\big( {#1} \big)}}
\newcommand{\activeptp}[1][\aG]{\mathsf{active}\big({#1}\big)}
\newcommand{\loopentrymsg}{\dag}
\newcommand{\loopexitmsg}{\ddag}
\newcommandx{\borderfn}[2][1=\aconfig,2=\aloop,usedefault=@]{
  \mathsf{border}_{{#2}}\ifempty{#1}{}{\big({#1}\big)}
}

\newcommand{\gs}{\textsf{\color{blue!60!green!80}gen\_server}}

\newcommand{\ggvisually}{
  $\begin{array}{c@{\qquad}c@{\qquad}c@{\qquad}c@{\qquad}c}
     % gint
     \begin{tikzpicture}[node distance=0.9cm and 0.4cm, every node/.style={scale=.7,transform shape}]
       \mkint{}{int}
       \mkgraph{int}{int};
       \node[above = .3cm of srcint, xshift=1cm, fill=green!50, opacity=.5, overlay, rectangle callout, callout absolute pointer={(srcint.east)}] {source node};
       \node[below = .3cm of sinkint, xshift=-1cm, fill=green!50, opacity=.5, overlay, rectangle callout, callout absolute pointer={(sinkint.west)}] {sink node};
     \end{tikzpicture}
     &
     % gseq
     \begin{tikzpicture}[node distance=.9cm and 0.4cm, every node/.style={scale=.7,transform shape}]
       \node[bblock] at (0,0) (g) {$\aG$};
       \node[node, below=of g] (s1) {};
       \node[bblock, below=of s1] (gp) {$\aG'$};
       \path[line,dotted] (g) -- (s1);
       \path[line,dotted] (s1) -- (gp);
     \end{tikzpicture}
     &
     % gpar
     \begin{tikzpicture}[node distance=.9cm and 0.4cm, every node/.style={scale=.7,transform shape}]
       \node[bblock] at (-.7,0) (g) {$\aG$};
       \node[bblock] at (.7,0)  (gp) {$\aG'$};
       \node[node, above=of g] (f) {};
       \node[node, below=of g] (j) {};
       \node[node, above=of gp] (fp) {};
       \node[node, below=of gp] (jp) {};
       \path[line,dotted] (f) -- (g);
       \path[line,dotted] (g) -- (j);
       \path[line,dotted] (fp) -- (gp);
       \path[line,dotted] (gp) -- (jp);
       \mkfork{f,fp}[fork][];
       \mkjoin{j,jp}[join][];
       \mkgraph{fork}{join};
       \node[above = .3cm of fork, xshift=1cm, fill=green!50, opacity=.5, overlay, rectangle callout, callout absolute pointer={(fork.east)}] {fork gate};
       \node[above = -.9cm of join, xshift=-1cm, fill=green!50, opacity=.5, overlay, rectangle callout, callout absolute pointer={(join.west)}] {join gate};
     \end{tikzpicture}
     &
     % gcho
     \begin{tikzpicture}[node distance=.9cm and 0.4cm, every node/.style={scale=.7,transform shape}]
       \node[bblock] at (-.7,0) (g) {$\aG$};
       \node[bblock] at (.7,0)  (gp) {$\aG'$};
       \node[node, above=of g] (f) {};
       \node[node, below=of g] (j) {};
       \node[node, above=of gp] (fp) {};
       \node[node, below=of gp] (jp) {};
       \path[line,dotted] (f) -- (g);
       \path[line,dotted] (g) -- (j);
       \path[line,dotted] (fp) -- (gp);
       \path[line,dotted] (gp) -- (jp);
       \mkbranch{f,fp}[fork][];
       \mkmerge{j,jp}[join][];
       \mkgraph{fork}{join};
       \node[above = .3cm of fork, xshift=1.2cm, fill=green!50, opacity=.5, overlay, rectangle callout, callout absolute pointer={(fork.east)}] {branch gate};
       \node[above = -.9cm of join, xshift=-1.2cm, fill=green!50, opacity=.5, overlay, rectangle callout, callout absolute pointer={(join.west)}] {merge gate};
     \end{tikzpicture}
     &
     % grec
     \begin{tikzpicture}[node distance=.5cm and 0.4cm, every node/.style={scale=.7,transform shape}]
       \node[bblock] at (-.5,0) (g) {$\aG$};
       \node[node, above=of g] (f) {};
       \node[node, below=of g] (j) {};
       \path[line,dotted] (f) -- (g);
       \path[line,dotted] (g) -- (j);
       \mkloop{f}{j};
       \mkgraph[.3cm]{entryf}{exitj};
       \node[above = .2cm of entryf, xshift=1.3cm, fill=green!50, opacity=.5, overlay, rectangle callout, callout absolute pointer={(entryf.east)}] {loop entry};
       \node[above = -.7cm of exitj, xshift=1.3cm, fill=green!50, opacity=.5, overlay, rectangle callout, callout absolute pointer={(exitj.west)}] {loop exit};
     \end{tikzpicture}
     \\
     \text{\scriptsize interaction}
     &
     \text{\scriptsize sequential}
     &
     \text{\scriptsize parallel}
     &
     \text{\scriptsize branching}
     &
     \text{\scriptsize iteration}
   \end{array}$
}
%\newcommand{\ts}{\toolid{TS}}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:

